Towards Scalable Physically Consistent Neural Networks: an Application to Data-driven Multi-zone Thermal Building Models

With more and more data being collected, data-driven modeling methods have been gaining in popularity in recent years. While physically sound, classical gray-box models are often cumbersome to identify and scale, and their accuracy might be hindered by their limited expressiveness. On the other hand, classical black-box methods, typically relying on Neural Networks (NNs) nowadays, often achieve impressive performance, even at scale, by deriving statistical patterns from data. However, they remain completely oblivious to the underlying physical laws, which may lead to potentially catastrophic failures if decisions for real-world physical systems are based on them. Physically Consistent Neural Networks (PCNNs) were recently developed to address these aforementioned issues, ensuring physical consistency while still leveraging NNs to attain state-of-the-art accuracy. In this work, we scale PCNNs to model building temperature dynamics and propose a thorough comparison with classical gray-box and black-box methods. More precisely, we design three distinct PCNN extensions, thereby exemplifying the modularity and flexibility of the architecture, and formally prove their physical consistency. In the presented case study, PCNNs are shown to achieve state-of-the-art accuracy, even outperforming classical NN-based models despite their constrained structure. Our investigations furthermore provide a clear illustration of NNs achieving seemingly good performance while remaining completely physics-agnostic, which can be misleading in practice. While this performance comes at the cost of computational complexity, PCNNs on the other hand show accuracy improvements of 17-35% compared to all other physically consistent methods, paving the way for scalable physically consistent models with state-of-the-art performance.

==> old_Conclusion.tex <==
\begin{comment}

    \section{Conclusion}
    \label{sec:conclusion}
    
This work presented the extension of single-zone PCNNs to the multi-zone setting, thereby providing control-oriented fully data-driven multi-zone building thermal models. The main idea is to treat parts of the inputs in a separate physics-inspired module to ensure given conditions are respected while the main dynamics are captured by a black-box module running in parallel and typically composed of NNs. 

The proposed PCNNs are theoretically grounded and respect the underlying physics by design and without engineering overhead. On the other hand, they outperformed state-of-the-art black-box methods in terms of accuracy on a case study, %analyzed in this work, 
hinting that the inductive bias introduced to ensure they follow some ground rules does not hinder their expressiveness. Furthermore, our investigations illustrated how classical PiNNs and LSTMs can find physically impossible shortcuts to fit the data well without respecting the underlying physical laws. This exemplifies the need to not solely consider the fit to the data as a measure of the quality of the fit of NNs but also to ensure that their predictions make sense, from the physical point of view, and calls for alternative solutions, like the proposed PCNNs. %, implying that a good fit of the data on its own is not a good measure of a model's quality in general.

Additionally, the proposed architectures showed significantly better performance than classical physically consistent data-driven methods, with improvements of $30$--$35\%$ and $17$--$22\%$ compared to a linear model, respectively a residual model. PCNNs are thus able to leverage the expressiveness of the NNs embedded in their black-box module to outperform existing physically grounded schemes. %, depending on which of the three architectures is used. 

In light of these results, PCNNs seem to pave the way for NN-based methods that are able to simultaneously provide state-of-the-art performance \textit{and} physical guarantees. We hence believe them to be an important step towards the safe deployment of NNs in real-world applications and hope to spark an interest both in the building modeling community and beyond. It would indeed be captivating to investigate the capabilities of PCNNs to model different buildings, incorporate additional nonlinearities in their black-box modules or rules in the physics-inspired ones, and tackle other complex physical systems.
%the proposed PCNN architectures attain state-of-the-art performance since they avoid the usual trade-off between the physical consistency and the accuracy of a model.
\end{comment}

%On the case study analyzed throughout this paper, the proposed PCNNs outperformed both classical gray-box and black-box methods in terms of accuracy. This shows the effectiveness of the inductive bias introduced in PCNNs to ensure they respect the underlying physical laws as it did not hinder their expressiveness compared to purely black-box approaches. Moreover, discarding all physically inconsistent methods, PCNNs attained significantly superior performance to gray-box models, with $35\%$ improvement over a classical linear model and $22\%$ over a residual one, which notably has a very similar architecture as PCNNs but a different training procedure. Altogether, PCNNs hence seem to be the most interesting models in practice, and one then needs to trade-off their accuracy with their computational complexity to select the most appropriate architecture for their application.

%While the case study investigated in this work exemplified the ability of PCNNs to handle the raw solar irradiation measurements, which have a highly nonlinear impact on the thermal behavior of the building, it is noteworthy that other nonlinear effects could be taken into account as well, typically involving the occupants of the building. Similarly, PCNNs could be useful in other fields where rudimentary physics-based models are available but nonlinear effects are hard to capture, i.e. anywhere gray-box models are used. For future work around PCNNs, it would hence be interesting to investigate their potential not only on different buildings, but also in dealing with other nonlinear impacts and in different applications.

==> old_Discussion.tex <==
    \section{Discussion}
    \label{sec:discussion}
    
%All the multi-zone PCNN models proposed and analyzed in this work were shown to be physically consistent with respect to power inputs, ambient temperatures, and initial conditions, making them interesting control-oriented building thermal model candidates. This was firstly derived theoretically and then visualized and analyzed numerically: 
Despite their black-box module, the proposed PCNNs respect the underlying physical laws at all times by construction and hence avoid the classical pitfall of NNs fitting patterns in the data with no physical meaning. In fact, the introduction of prior knowledge was beneficial in the presented case study, with PCNNs outperforming their unconstrained counterparts, namely LSTMs and PiNNs. Our analyses clearly illustrate the danger of solely relying on a measure of "fit to the data" to assess the quality of a model when dealing with NNs, something often overlooked. We could indeed train LSTMs and PiNNs to attain very good performance despite being completely oblivious to the underlying physical laws and thus useless in practice. One should thus be careful when modeling physical systems with NNs and ensuring that their predictions make sense, for example using schemes similar to the ones grounding PCNNs in the underlying physics to ensure the model does not learn a non-physical shortcut to the solution. Altogether, our findings hence support the current trend to incorporate inductive biases in DL models to alleviate the infamous brittleness and generalization issues.
 %One the other hand, we observed PCNNs to perform significantly better than classical physics-based gray-box methods, obtaining $40\%$, respectively $17\%$, lower errors than a linear, respectively a residual models. Altogether, PCNNs thus seem to be able to avoid the usual trade-off between accuracy and physical consistency often observed in modeling by attaining state-of-the-art accuracy without loosing the desired physical consistency. 
 
Focusing on the proposed physically consistent PCNN architectures, only minor differences could be observed. While X-PCNNs seem to attain the best performance in general, they require the most training resources, whereas S-PCNNs attain slightly worse results but significantly reduce the computational burden. Compared to the other two methods, M-PCNNs strike a middle ground, with good performance, robust to the choice of a random seed, attained with a medium amount of resources. Interestingly, all of them clearly outperform the other two physically consistent methods, making them state-of-the-art thermal building models with physical guarantees.

%Among the three proposed architectures, all of which stay physically consistent at all time by construction, it seems that only minor differences in performance can be attained depending on the random seed used at each time. From our analyses, the X-PCNN architecture presented a slight advantage compared to the other two models in terms of accuracy, but it was simultaneously the most computationally intensive method to train, so that we get a trade-off between the computational load and the performance of PCNNs at the end of the day. 

Remarkably, while only solar irradiation measurements and time information were fed to the black-box module of PCNNs throughout this study, showcasing the ability of the proposed approach to handle highly nonlinear effects, other inputs could be integrated in a straightforward manner. This might typically include the impact of the occupants or additional external conditions. Similarly, additional physics-based components could extend or replace the current physics-inspired module to capture different effects, for example, to capture the influence of window openings. This work hence only presented a few ideas to use the very modular PCNN architecture in the case of thermal modeling, but it might be extended further, or applied to other physical systems, as mentioned in Section~\ref{sec:PCNN}.

%As for single-zone PCNNs, these remarks naturally extend to other fields, beyond thermal modeling, where simplified physical laws can be complemented by a black-box module to model complex phenomena.

%Note that the proposed architectures are currently power input-affine, so that it is straighforward to optimize the energy consumption of a building subject to temperature constraints, making these PCNNs ideal simulation environments for the development of intelligent controllers.

Lastly, one should keep in mind all the results in Section~\ref{sec:results} were obtained on a specific case study and might have been impacted by the random seeds used despite our best efforts to cancel these effects through multiple runs. %Importantly, while the theory would not change for another case study, the performance of all the models would. 
Nevertheless, based on the results presented in this work, we can expect PCNNs to outperform the other physically consistent methods on various case studies, so that they should remain the best modeling choice in general, even if classical black-box methods might attain a better accuracy on different data sets.


